LTBD: Learnable Trust-Boundary Delimiters for Prompt Injection Defense

Large language models (LLMs) perform remarkably well on complex tasks, yet remain highly vulnerable to prompt injection attacks, where malicious instructions embedded in external data can override user intent. Existing defenses remain limited by model fine-tuning requirements, vulnerability to adaptive attacks, or reliance on brittle handcrafted prompts. We argue that a fundamental source of this vulnerability is the lack of an explicit representation of trust provenance. To address this, we introduce Learnable Trust-Boundary Delimiters (LTBD), a lightweight defense that explicitly encodes trust boundaries in the input while keeping the LLM parameters unchanged. LTBD uses a small number of learnable delimiters to distinguish trusted user instructions from untrusted external data, enabling the model to better respect the intended trust hierarchy. Experimental results show that LTBD substantially outperforms inference-time defenses and performs competitively with training-based approaches, while preserving benign-task utility and introducing negligible inference overhead. In particular, LTBD achieves 0.00% ASR on AlpacaFarm and only 0.11-0.19% ASR on TaskTracker. LTBD also remains effective under adaptive attacks, where adversaries have full knowledge of the defense and explicitly attempt to bypass it.

==> method_old.tex <==
\section{Method}
\label{method}
\subsection{Problem Formulation}

We consider an LLM application that jointly processes task instructions and external data, with the input structure illustrated in Fig.~\ref{fig:prompt_injection}.
\begin{figure}[h]
    \centering    \includegraphics[width=1.0\columnwidth]{fig1.pdf}
    \caption{Input structure and prompt injection attack in an LLM-integrated application.}
    \label{fig:prompt_injection}
\end{figure}
\begin{figure*}[t]
    \centering    \includegraphics[width=1.0\textwidth]{fig2.pdf}
    \caption{Overview of the proposed method. (a) Without defense, prompt injections embedded in external data may steer the LLM away from the original task. (b) Four Learnable Trust-Boundary Delimiters mark the boundaries of trusted instructions and untrusted data. The base LLM remains frozen, and only the delimiter embeddings are optimized using our training objective.}
    \label{fig:framework}
\end{figure*}
Given an original trusted task instruction $I$ and external data $D$, an attacker injects a malicious instruction $A$ into the data, yielding
\begin{equation}
D' = D \oplus A,
\end{equation}
where $\oplus$ denotes inserting the attack instruction into the original data. For a benign input $(I,D)$, the model should follow task instruction $I$ and perform the specified task over data $D$. For an attacked input $(I,D')$, even though $D'$ contains attack content $A$ with complete instruction semantics, the model should still treat it as part of the data to be processed rather than as a new instruction with the same behavioral authority. We therefore formulate prompt injection defense as a trust-boundary modeling problem: explicitly distinguishing the trusted instruction region from the untrusted data region and providing the frozen model with structured trust information.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.95\textwidth]{fig2.png}
%     \caption{Overview of the proposed method. (a) Without defense, prompt injections embedded in external data may steer the LLM away from the original task. (b) We introduce four Learnable Trust-Boundary Delimiters to explicitly mark the beginning and end of trusted instructions and untrusted data. The base LLM remains frozen, and only the embeddings of the four delimiters are optimized using the constructed training objective.}
%     \label{fig:framework}
% \end{figure*}

\subsection{Learnable Trust-Boundary Delimiters}

% StruQ~\cite{chen2025struq} and DefensiveToken~\cite{chen2025defending} demonstrate the effectiveness of structured input separation and lightweight learnable representations, respectively, for prompt injection defense. Inspired by these observations, 
We introduce four learnable boundary delimiters while freezing the base model parameters. The delimiters are placed at the beginning and end of the trusted task instruction and untrusted external data, and only their embeddings are optimized, explicitly associating the trainable representations with input trust boundaries.

Specifically, we introduce four special tokens
$\mathcal{T}=\{t_{\mathrm{IB}},t_{\mathrm{IE}},t_{\mathrm{DB}},t_{\mathrm{DE}}\}$,
which mark the beginning and end of the trusted instruction region and the untrusted data region. Their embedding matrix is denoted by $T\in\mathbb{R}^{4\times e}$, where $e$ is the token embedding dimension of the base model. Given a trusted instruction $I$ and external data $\hat{D}$, where $\hat{D}$ can be benign data $D$ or attacked data $D'=D\oplus A$, the model input with the four delimiters is represented as
\begin{equation}
x_T=
[t_{\mathrm{IB}};I;t_{\mathrm{IE}};
 t_{\mathrm{DB}};\hat{D};t_{\mathrm{DE}}],
\label{eq2}
\end{equation}
where semicolons denote sequence concatenation, and the four delimiters mark the beginning and end of the trusted instruction and untrusted data regions. During training, the base model parameters $\theta$ remain frozen, and only the embedding matrix $T$ is jointly optimized using supervised cross-entropy and an auxiliary preference constraint. For attacked samples, the training objective is
% {\small
% \begin{equation}
% \begin{aligned}
% \mathcal{L}
% &=
% \mathcal{L}_{\mathrm{CE}}
% +\lambda\mathcal{L}_{\mathrm{pref}} \\
% &=
% -\log p_{\theta,T}(y^{+}\mid x_T) 
% % &\quad
% -\lambda\log\sigma\Big[
% \beta\Big(
% \log p_{\theta,T}(y^{+}\mid x_T) 
% % &\qquad\qquad
% -\log p_{\theta,T}(y^{-}\mid x_T)
% \Big)\Big],
% \end{aligned}
% \label{eq:loss}
% \end{equation}}
{\small
\begin{equation}
\begin{aligned}
\mathcal{L}
&= \mathcal{L}_{\mathrm{CE}}
 + \lambda \mathcal{L}_{\mathrm{pref}} \\
&= -\log p_{\theta,T}(y^{+}\!\mid x_T)
-\lambda \log \sigma\!\left[
\beta \log
\frac{p_{\theta,T}(y^{+}\!\mid x_T)}
     {p_{\theta,T}(y^{-}\!\mid x_T)}
\right],
\end{aligned}
\label{eq:loss}
\end{equation}}
where $y^{+}$ is the reference response corresponding to the original benign input, $y^{-}$ is the negative response generated by the undefended model on the attacked input, $\lambda$ is the weight of the auxiliary preference loss, $\beta$ is a scaling factor, and $\sigma(\cdot)$ is the sigmoid function. For benign samples, we set $\mathcal{L}_{\mathrm{pref}}=0$ and compute only the cross-entropy loss.

To optimize the above objective, following StruQ~\cite{chen2025struq}, we construct a defensive training dataset $\mathcal{D}_{\mathrm{def}}$ from an 
instruction-tuning dataset $\mathcal{D}$. First, following prior work~\cite{chen2025defending,chen2025meta}, we self-label each original benign input $(I,D)\in\mathcal{D}$ using the undefended base model to obtain a reference response $y^{+}=f_{\theta}(I,D)$. Subsequently, We  keep half of the samples unchanged and apply three prompt injection variants with equal probability to the remaining samples with non-empty external data, constructing attacked samples $(I,D')$. Whether the training input remains $(I,D)$ or is transformed into $(I,D')$, the same $y^{+}$ generated from the original benign input is used as the cross-entropy supervision target, encouraging the model to preserve the original task behavior in the presence of injected content.

For attacked samples, we further use the undefended base model to generate a negative response $y^{-}=f_{\theta}(I,D')$ and pair it with the reference response $y^{+}$. The auxiliary preference loss encourages a higher relative probability for $y^{+}$ than for $y^{-}$, strengthening the model's preference for the reference task behavior. Accordingly, the defensive training dataset is uniformly represented as
$\mathcal{D}_{\mathrm{def}}=\{(I_i,\hat{D}_i,y_i^{+},y_i^{-})\}_{i=1}^{N}$,
where $N$ is the number of training samples. A benign sample is represented as $(I,D,y^{+},\varnothing)$, while an attacked sample is represented as $(I,D',y^{+},y^{-})$. Algorithm~\ref{alg:training} summarizes the complete training procedure.

% \begin{algorithm}[t]
% \caption{Training Learnable Trust-Boundary Delimiters}
% \label{alg:training}
% \begin{algorithmic}[1]
% \REQUIRE Base model $f_{\theta}$ parameterized by $\theta$, instruction-tuning dataset $\mathcal{D}$
% \ENSURE Embedding matrix $T$ of the trust-boundary delimiters

% \STATE Freeze the base model parameters $\theta$
% \STATE Construct the four-tuple training set $\mathcal{D}_{\mathrm{def}}$ via self-labeling, prompt injection, and negative-response generation
% \STATE Initialize $T\in\mathbb{R}^{4\times e}$, with each element independently sampled from $\mathcal{N}(0,1)$

% \FOR{each batch $\mathcal{B}\subseteq\mathcal{D}_{\mathrm{def}}$}
%     \STATE Construct $x_T$ for each sample according to Eq.~\eqref{eq2}
%     \STATE Compute the joint loss according to Eq.~\eqref{eq:loss}
%     \STATE Update $T$ using gradients of the loss
% \ENDFOR

% \RETURN $T$
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[t]
\caption{\footnotesize Training Learnable Trust-Boundary Delimiters}
\label{alg:training}
{\footnotesize
\begin{algorithmic}[1]
\REQUIRE Base model $f_{\theta}$, instruction-tuning dataset $\mathcal{D}$
\ENSURE Trust-boundary delimiter embeddings $T$

\STATE $y^{+}\leftarrow f_{\theta}(I,D),\ \forall(I,D)\in\mathcal{D}$
\STATE Obtain attacked samples $(I,D')$ with
$D'=D\oplus A$, where $A$ denotes an injected instruction
\STATE $y^{-}\leftarrow f_{\theta}(I,D')$ for attacked samples
\STATE $\mathcal{D}_{\mathrm{def}}
\leftarrow\{(I_i,\hat D_i,y_i^{+},y_i^{-})\}_{i=1}^{N}$,
where $\hat D_i\in\{D_i,D'_i\}$

\STATE Add $\mathcal{T}=
\{t_{\mathrm{IB}},t_{\mathrm{IE}},t_{\mathrm{DB}},t_{\mathrm{DE}}\}$
to the vocabulary
\STATE Initialize $T\in\mathbb{R}^{4\times e}$ with
$T\sim\mathcal{N}(0,I)$
\STATE Freeze $\theta$ and optimize only $T$

\FOR{each $(I,\hat D)\in\mathcal{D}_{\mathrm{def}}$}
    \STATE $x_T\leftarrow
    [t_{\mathrm{IB}};I;t_{\mathrm{IE}};
    t_{\mathrm{DB}};\hat D;t_{\mathrm{DE}}]$
    \STATE $\mathcal{L}
    \leftarrow\mathcal{L}_{\mathrm{CE}}+ \lambda \mathcal{L}_{\mathrm{pref}}$ as Eq.~\eqref{eq:loss},
    \STATE Update $T$ using $\nabla_T\mathcal{L}$
\ENDFOR

\RETURN $T$
\end{algorithmic}}
\end{algorithm}

==> related_work.tex <==
\section{Related Work}

% \textbf{Prompt Injection Defenses.}
Prompt injection attacks manipulate LLMs through malicious instructions embedded in untrusted data, causing them to ignore legitimate tasks and follow attacker-specified behaviors, and have become a major security concern for LLM-integrated applications. Existing defenses mainly fall into two categories: test-time defenses and training-based defenses.

Test-time defenses introduce defensive prompts or additional control signals to guide models toward legitimate instructions while ignoring malicious injections. Among them, Reminder~\cite{yi2025benchmarking} adds a safety reminder before untrusted data to explicitly instruct the model to ignore malicious instructions contained within it; Sandwich~\cite{learnprompting2023sandwich} adopts an ``instruction--data--safety reminder'' structure and reiterates the original task after the data; TextGrad~\cite{yuksekgonul2025optimizing} performs black-box text optimization to search for more effective discrete defensive prompts without accessing model gradients. DefensiveToken~\cite{chen2025defending} instead keeps the base model frozen, optimizes only the embeddings of a small number of newly introduced tokens, and prepends them to the input at inference time to provide lightweight defense through learnable continuous representations. These methods do not require updating the base model parameters, but their effectiveness largely depends on how the model responds to defensive prompts or control signals.

Training-based defenses directly modify model behavior through security-oriented fine-tuning or preference optimization. StruQ~\cite{chen2025struq} combines structured queries with supervised fine-tuning, using dedicated delimiters to distinguish task instructions from user data and training the model to follow only the requirements in the instruction region. SecAlign~\cite{chen2025secalign} adopts preference optimization to increase the preference for legitimate-task responses over attack-induced responses, thereby improving instruction-following robustness under prompt injection. These methods learn secure behavior from the perspectives of structured separation and response preference, but typically require updating the base model parameters.

Our method combines structured separation with lightweight representation learning by explicitly associating learnable representations with the trust boundaries between trusted instructions and untrusted data. Unlike the prefix-based defensive tokens in DefensiveToken, our learnable delimiters are placed at the structural boundaries of regions with different trust levels. Unlike training-based defenses, the base LLM remains frozen and only the embeddings of the newly introduced delimiters are optimized.
